Variational Message Passing with Structured Inference Networks

Recent efforts on combining deep models with probabilistic graphical models are promising in providing flexible models that are also easy to interpret. We propose a variational message-passing algorithm for variational inference in such models. We make three contributions. First, we propose structured inference networks that incorporate the structure of the graphical model in the inference network of variational auto-encoders (VAE). Second, we establish conditions under which such inference networks enable fast amortized inference similar to VAE. Finally, we derive a variational message passing algorithm to perform efficient natural-gradient inference while retaining the efficiency of the amortized inference. By simultaneously enabling structured, amortized, and natural-gradient inference for deep structured models, our method simplifies and generalizes existing methods.

==> svmp.tex <==
In the previous section, we proposed a conjugate-structure inference network. Now, we describe a variational message-passing (VMP) algorithm to perform efficient inference with it. Our goal is to maximize the following lower bound:
\begin{align}
\log p(\vy) \geq \myexpect_{q(\modl|\lambda)q(x|y,\infe)} \sqr { \log \frac{p(\vy,\vlat, \vmodl)}{q(\vlat|\vy,\vinfe) q(\vmodl|\vlambda) } } & := L(\vinfe, \vlambda), \label{eq:elbo}
\end{align}
where $\vlambda$ is the parameter of the variational distribution $q(\vmodl|\vlambda)$. While it would be possible to also put a prior on the inference network parameters $\vinfe$, we assume them to be deterministic. As the inference network can be viewed to just be a tool to efficiently learn the model parameters, it does neither seem to be important to put a prior on $\vinfe$, nor do we think it adds any advantage. Note that this varitational lower bound is very similar to the bound in VAEs \citep{kingma2013auto}. The difference is that our bound additionally includes the term $q(\vmodl\given\vlambda)$ which is not needed in VAE. 

A straightforward approach to maximise this bound is to use a stochastic-gradient (SG) methods such as RMSprop or Adam. While these methods are suitable for estimating the deterministic parameters $\vinfe$, they may be inefficient to estimate $\vlambda$. This is because SG methods are not suited for optimizing variational parameters (see a discussion in \cite{hoffman2013stochastic}). 

%TODO conjugacy
A preferred way to optimize with respect to $\vlambda$ is to use natural-gradient methods such as stochastic variational inference (SVI) \citep{hoffman2013stochastic}. 
SVI enables variational inference with large-scale datasets and can be viewed as a stochastic extension of the VMP algorithm \citep{winn2005variational}. VMP gains its computational efficiency by exploiting conditional independencies to decompose the overall optimisation into a set of local computations. Within the VMP framework, updating a node's posterior belief only requires information about the neighboring nodes in the model graph. In conjugate-exponential models, this leads to a very simple closed-form updates that correspond to a step of unit length in the direction of the natural-gradient \citep{paquetconvergence}. For optimising variational parameters, SG methods cannot exploit these nice properties and might converge more slowly.

Thus, an alternative to SG methods is to use natural-gradients for both $\vinfe$ and $\vlambda$. However, this is computationally expensive since computing the natural-gradient of a deterministic parameter requires the Fisher matrix. We could also simply apply natural-gradient updates to $\vlambda$ and use SG methods for $\vinfe$, but this approach is not principled and the step-sizes might be difficult to tune due to the interaction between these different types of updates. 

As opposed to these naive ideas, we propose a principled approach that automatically recovers SG updates for the deterministic $\vinfe$ as a special case, while enabling natural-gradient updates for $\vlambda$. To do so, we use the conjugate-computation variational inference algorithm (CVI) \citep{khan2017conjugate} that generalises VMP and SVI for the convenient use of non-conjugate terms. While we can apply CVI to learn the stochastic model parameters $\vmodl$, we cannot directly use it for the deterministic inference network parameters $\vinfe$. We will first explain how we use a recent extension of CVI to deal with the inference network and then present the updates for the stochastic parameters.


\subsection{Deterministic Parameters} \label{sec:detparams}
To allow the use of inference networks, we associate $\vinfe$ with a Gaussian distribution $q(\vinfe) := \gauss(\vinfe|\vmu_\infe,\diag(\vsigma_\infe^2))$ where $\vmu_\infe$ and $\vsigma_\infe$ are vectors of mean and standard deviation. We choose $q(\vinfe)$ to be a  mean-field approximation (i.e. the covariance matrix is diagonal) because the number of parameters for DNNs is typically large. Given this distribution, we maximize the following lower bound:
\begin{align}
	\bar{\mathcal{L}}(\vmu_\phi,\vSigma_\phi,\vlambda) := \myexpect_{q(\phi)} [\mathcal{L}(\vlambda,\vphi)].\label{eq:elboVO}
\end{align}

This approach is known as variational optimization (VO) \citep{staines2012variational} and it works due to the following inequality: $\max \mathcal{L}(\vinfe,\vlambda) \ge \myexpect_{q(\infe)} [\mathcal{L}(\vinfe,\vlambda)]$, i.e., the maximum of a function is lower bounded by the function's expectation. Therefore, maximizing the expectation also maximizes the function. While the variational optimization algorithm converges, the variance $\vsigma_\infe^2$ eventually shrinks to zero, which is why the result is a local minima of $\mathcal{L}$ even though we optimize $\bar{\mathcal{L}}$.

{\bf Update for $q(\vphi|\vmu_\phi,\vsigma_\phi^2)$: }The good news is that CVI has recently been made applicable to variational optimization, resulting in the variational adaptive-newton method (VAN) \citep{khan2017van}. VAN is a blackbox optimization method that uses the distribution $q(\vinfe)$ to enable learning via exploration, i.e., it uses the variance $\vsigma_\infe^2$ to avoid local minima. \citet{khan2017van} show that applying CVI to VO results in the following second-order SG updates:
\begin{align}
	\sigma_\infe^{-2} &\leftarrow \sigma_\infe^{-2} + 2\beta_t\myexpect_{q(\phi)} \sqr{\nabla^2_{\infe\infe}\mathcal{L}(\vlambda,\vphi)}\label{eq:updateVAN1}\\
	\mu_\infe &\leftarrow \mu_\infe - \beta_t\sigma_\infe^2\myexpect_{q(\phi)} \sqr{\nabla_{\infe} \mathcal{L}(\vlambda,\vphi)},
	\label{eq:updateVAN2}
\end{align}
%TODO make equal to functions used in algorithm 1
%TODO include stochasticity
where the gradient in \eqref{eq:updateVAN1} as well as the Hessian in \eqref{eq:updateVAN2} can be approximated using the reparameterization trick (see section 4 in \citet{khan2017van}). The gradient computation in our method is therefore very similar to the gradient computation in VAE \citep{kingma2013auto} (this is further highlighted in Algorithm \ref{alg:updateSAN}). 
Also, our updates are very similar to typical adaptive-gradient methods where the variance $\sigma_\infe^2$ acts as scaling vector in the update for the mean $\mu_\infe$. In fact, they are closely related to AdaGrad \cite{Duchi2011adaptive}. Learning deterministic parameters using our method is therefore very similar to applying AdaGrad to VAE. 

Note that if we choose not to put a prior on $\vmodlNN$, its updates are the same as for $\vinfe$. This is what we do in Algorithm \ref{alg:updateSAN} for simplicity, i.e., we assume $\vmodlNN$ to be deterministic and update it together with the inference network parameters. Below, we still show how to update $\vmodlNN$ in the stochastic case.
%To derive these updates, we note that the neighbors of $\vphi$ are the factors that use $\vlat$, i.e., $p(\vy|\vlat,\vmodlNN)$, $p(\vlat|\vmodlGM)$ and $q(\vlat|\vy,\vinfe)$ itself. 
%\begin{align}
%   \bar{\mathcal{L}}(\vmu_\phi,\vsigma_\phi^2) = \myexpect_{q(\theta)q(\phi)q(x|y,\phi)}\sqr{\log \frac{p(\vy|\vlat,\vmodlNN) p(\vlat|\vmodlGM)}{q(\vlat|\vy,\vinfe)} }
%\end{align}
%Since the distribution is Gaussian we can use updates very similar to \eqref{eq:update1}-\eqref{eq:update2}. To compute the gradient we can use reparameterization trick since a sample from $q(\vlat|\vy,\vinfe)$ is a function of $\vmu_\phi$ and $\vsigma_\phi^2$. The updates again resemble adaptive-gradient methods and can be easily obtained. 


\subsection{Stochastic Parameters}

{\bf Update for $q(\vmodlGM|\vlamGM)$: } We assume that $p(\vmodlGM)$ and $p(\vlat|\vmodlGM)$ are exponential family distributions and conjugate to each other (although the algorithm can easily be modified when the relationship is non-conjugate). Conjugacy implies that prior and likelihood can be expressed in the same exponential family form with respect to $\vmodlGM$ (e.g., see Section 2 in \cite{khan2017conjugate}):
\begin{align}
   p(\vmodlGM) &=  h(\vmodlGM)\exp\sqr{\ang{\vT(\vmodlGM), \veta} - A(\veta)} \label{eq:pgm_prior} \\
   p(\vlat|\vmodlGM) &= \exp\sqr{\ang{\vT(\vmodlGM), \veta_{x\theta}(\vlat)} -f_x(\vlat)} , \label{eq:conjexp1}
\end{align}
where $\veta$ is the natural parameter, $\vT$ is the sufficient statistics, $\ang{\cdot,\cdot}$ is an inner product, $h$ is the base measure, $A(\veta)$ is the log-partition function, and $\veta_{x\theta}$ and $f_x$ are functions that depend on $\vlat$ only.
In our graphical model, the only factors that involve $\vmodlGM$ are $p(\vlat|\vmodlGM)$ and $p(\vmodlGM)$. Therefore, using Algorithm 2 of \cite{khan2017conjugate}, we can write the natural-gradient update for the approximate posterior $q(\vmodlGM|\vlamGM)$ as follows:
\begin{align}
\vlamGM \leftarrow (1-\beta_t) \vlamGM + \beta_t \,\, \myexpect_{q(x|y,\phi)q(\phi)}\sqr{ \veta + \veta_{x\theta}(\lat)} \label{eq:svi_update}
\end{align}
where $\beta_t>0$ is the step-size in iteration $t$.
To compute the expectation we first generate samples $\vlat_*$ from the inference network. Given these samples, the computation of the message $\veta_{x\theta}$ is equivalent to performing variational inference in the model $p(\vlat_*,\vmodlGM)$ which can be done using standard methods such as SVI and VMP for which we can reuse existing software. Therefore, the design of our inference network results in a simple and efficient update for our model's PGM prior that does not require any gradient computations.

{\bf Update for $q(\vmodlNN|\vlamNN)$: } We assume that the prior of all elements of $\vmodlNN$ is a Gaussian with mean $\mu_0$ and variance $\sigma_0^2$. Since the prior is Gaussian, we also choose the posterior approximation $q(\vmodlNN|\vlamNN)$ to be Gaussian and because the number of parameters for DNNs is usually large, we use a mean-field approximation (i.e., $\vlambda_{{NN}} = \{\vmu, \vsigma\}$). For simplicity, we show updates only for the $i$'th element of $\vmodlNN$. We denote the mean and variance of this element by $\mu_i$ and $\sigma_i^2$ respectively.

We first note that the only factors in our bayesian network \eqref{eq:joint} involving $\vmodlNN$ are $p(\vmodlNN)$ and $p(\vy|\vx,\vmodlNN)$. Because of the non-linearity introduced by the neural netowork, the true posterior distribution $p(\vmodlNN\given\vy)$ is not of the same form as the prior $p(\vmodlNN)$. Therefore, prior and likelihood are not conditionally conjugate and applying Algorithm 2 of \cite{khan2017conjugate} results in an SG update:
\begin{align}
   \sigma_i^{-2} &\leftarrow (1-\beta) \sigma_i^{-2} - \beta  \sqr{1/\sigma_0^2 + \nabla_{\sigma_i^2} \myexpect_{q(\theta)q(\phi)q(x|y,\phi)}\rnd{\log p(\vy|\vlat,\vmodlNN)} } \label{eq:update1} \\ 
   \mu_i &\leftarrow \mu_i - \beta \sigma_i^2 \sqr{\mu_0/\sigma_0^2 + \nabla_{\mu_i} \myexpect_{q(\theta)q(\phi)q(x|y,\phi)}\rnd{\log p(\vy|\vlat,\vmodlNN)} }   \label{eq:update2}
\end{align}
%These updates are very similar to a typical adaptive-gradient method where the variance $\sigma_i^2$ acts as scaling vector in the update for the mean $\mu_i$. There are three differences: First, both updates involve a regularization term, namely $1/\sigma_0^2$ and $\mu_0/\sigma_0^2$. Second, the gradient with respect to the variance is computed. Third, the gradients are computed at a location randomly sampled from $q$. Despite these differences, our experiments show that these updates converge at a rate very similar to adaptive gradient methods. 

Note that these updates are very similar to the VO-updates for $\vinfeNN$ \eqref{eq:updateVAN1}-\eqref{eq:updateVAN2}. The main difference is that the updates for $\vmodlNN$ involve regularization terms, namely $1/\sigma_0^2$ and $\mu_0/\sigma_0^2$. The reason is that we do not define any prior over $\vinfe$ and that $q(\vinfe)$ does not appear \textit{inside} the expectation in \eqref{eq:elboVO}. 


\subsection{Summary of the method}

%\begin{algorithm}[t]
%\caption{Update for SAN}
%\label{alg:updateSAN}
%\hspace*{\algorithmicindent} \textbf{Require: }  Parameter $\veta_\text{PGM}$ \eqref{eq:pgm_prior}, Function $\veta_{\theta}(\cdot)$ \eqref{eq:conjexp1}
%
%\begin{algorithmic}[1]
%
%    \FOR{Iteration $t=1,2,3,\ldots$,}
%	\STATE Randomly pick a data point $\vy_n$
%	
%	\STATE Sample global parameters $\vmodlGM$ and $\vdtrmc := \crl{\vmodlNN, \vinfe}$ \label{algstep:sampleglob}
%	
%		$\vtheta^{*}_\text{PGM} \sim q(\vtheta_{PGM} | \vlambda_\text{PGM})$
%		
%		$\vdtrmc^{*} \sim \gauss( \vdtrmc | \vmu_{\dtrmc}, \vsigma^2_{\dtrmc} ) $
%   
%   
%	\STATE Sample local latent variable from the inference network (as in VAE)
%	
%		$\vx_n^{*} \sim q(\vx_n|\vy_n, \vphi^{*} )$
%    
%    
%	\STATE Update $q(\vmodlGM|\vlambda_\text{PGM})$ using eq.\ref{eq:svi_update} (perform VI in PGM part of model using samples $\vx_n^{*}$)
%	
%%		$\vlambda_\text{PGM} \leftarrow  (1-\beta) \vlambda_\text{PGM} + \beta N   \sqr{ \veta_\text{PGM} + \veta_{\theta}( \vx_n^{*} ) }$    
%
%
%	\STATE Compute gradient w.r.t. $\vdtrmc$ (as in VAE)
%	
%		$\vg \leftarrow  \nabla_{\dtrmc } \log p(\vy_n|\vx^{*}_n, \vtheta^{*}_\text{NN} ) + \log \frac{ p(\vy_i|\vtheta_\text{PGM})}{ q(\vx_n|\vy_n, \vphi_\text{NN}) } \bigg\rvert_{\vdtrmc = \vdtrmc^{*}  }$
%

%	\STATE Update gradient (additional terms of our method compared to VAE)
%
%		$\vg \leftarrow  \vg + \nabla_{\dtrmc } \sqr{-\log p(\vx^{*}_n | \vphi_\text{PGM}) + \log \mathcal{Z}(\vphi) } \bigg\rvert_{\vdtrmc = \vdtrmc^{*}  } $
%
%	\STATE Perform adaptive-gradient update \eqref{eq:updateVAN1}-\eqref{eq:updateVAN2}

%		$\vsigma_\dtrmc^{-2} \leftarrow \vsigma_\dtrmc^{-2} + \beta \vg \odot \vg$
%
%		$\vmu_\dtrmc \leftarrow \vmu_\dtrmc - \beta \vsigma_\dtrmc^{2} \odot \vg $
%
%    \ENDFOR
%\end{algorithmic}
%\end{algorithm}

The method of \cite{khan2017conjugate} is guaranteed to converge under stochastic SVI-like updates where a local variable update is followed by the update of global variable. Since we are using an inference network for the local variables, this is equivalent to generating samples from $q(\vlat|\vy,\vinfe)$. Using the generated samples we can either perform the above three updates in parallel of use a sequential mode. It is also allowed to randomly pick a global variable and update them. We end this section with the continuation of our latent GMM example:

\begin{tabular}{|p{0.97\textwidth}}
{\bf GMM Example (VMP updates) :} For simplicity, we assume that $\vtheta_\text{NN}$ are deterministic parameters, which is similar to VAE. As defined in Algorithm \ref{alg:updateSAN}, we first generate samples of the global parameters $ \vdtrmc^* = \crl{\vmodlNN^*, \vinfe^*}$ and $\vtheta^{*}_\text{PGM}$.  After that, we generate the messages from the inference network, i.e., we sample $ z_n^{*} \sim (z_n|\vy_n,\vphi^{*})$ and $\vx_n^{*} \sim q(\vx_n|z_n^{*}, \vy_n,\vphi^{*})$ \eqref{eq:qz}-\eqref{eq:qx}.

It can be shown that the terms involving $\vmodlGM$ in our lower bound \eqref{eq:elbo} are very similar to the lower bound maximised in the M-step of the variational GMM-EM algorithm described in \cite{bishop2006pattern}. We therefore choose the same conjugate prior as in this algorithm: $p(\vmodlGM) = p(\vpi)\prod_{k=1}^{K} p(\vpsi_{k})$, where $p(\vpi)$ is a $K$-dimensional Dirichlet distribution and $p(\vpsi_{k} )$ is a Normal-Wishart distribution. Given the samples $z_n^{*}, x_n^{*}$, we apply the M-step updates given in eq.10.57-10.63 in \citet{bishop2006pattern} for computing $\myexpect_{q(x|y,\phi)q(\phi)}\sqr{ \veta + \veta_{x\theta}(\lat)}$ in \eqref{eq:svi_update}.

We use the variational optimization approach described in section \ref{sec:detparams} to optimize the deterministic parameters, i.e., $q(\vdtrmc )=\gauss(\vdtrmc| \vmu_\dtrmc, \vsigma^2_\dtrmc )$.
Similar to the VAE updates, we apply the re-parametrization trick to compute the gradient messages for updating $\crl{ \vmu_\dtrmc, \vs_\dtrmc}$ \eqref{eq:updateVAN1}, \eqref{eq:updateVAN2}.
\end{tabular}





%\begin{algorithm} 
%
%\caption{Update for SAN}
%\label{alg:updateSAN}
%\hspace*{\algorithmicindent} \textbf{Require: }  Parameter $\veta_\text{PGM}$ (eq.\ref{eq:pgm_prior}), Function $\veta_{\theta}(\cdot)$ (eq.\ref{eq:conjexp1}) 
%
%\begin{algorithmic}[1]
%
%    \FOR{Iteration $t=1,2,3,\ldots$,}
%	\STATE Randomly pick a data point $n$
%	
%   \STATE Sample $\vtheta_\text{NN}$, and $\vphi$
%   
%   $\vtheta^{*}_\text{NN} \sim \gauss( \vtheta_{\theta_\text{NN}} | \vmu_{\theta_\text{NN}}, \vsigma^2_{\theta_\text{NN}} )$
%
%   $\vphi^{*} \sim \gauss( \vphi | \vmu_{\phi}, \vsigma^2_{\phi} ) $
%   
%   \STATE Sample $\vtheta_\text{PGM}$
%   
%   $\vtheta^{*}_\text{PGM} \sim q(\vtheta_{PGM} | \vlambda_\text{PGM})$
%   
%   \STATE Sample from the inference network
%    
%    $\vx_n^{*} \sim q(\vx_n|\vy_n, \vphi^{*} )$
%    
% \STATE Update $q(\vtheta_\text{PGM}|\vlambda_\text{PGM})$ using eq.\ref{eq:svi_update}
%    
%$\vlambda_\text{PGM} \leftarrow  (1-\beta) \vlambda_\text{PGM} + \beta N   \sqr{ \veta_\text{PGM} + \veta_{\theta}( \vx_n^{*} ) }$    
%
%\STATE Compute gradient w.r.t. $\vtheta_\text{NN}$ using the same method as in VAE
%
%$\vg_{\theta_\text{NN}} \leftarrow  \nabla_{\theta_\text{NN}} \log p(\vy_i|\vx_i^{*}, \vtheta_\text{NN} ) \bigg\rvert_{\vtheta_\text{NN}= \vtheta^{*}_\text{NN} }$
%
%\STATE Compute gradient w.r.t. $\vphi$ using the same method as in VAE
%
%$\vg_{\phi} \leftarrow  \nabla_{\phi } \log p(\vy_n|\vx^{*}_n, \vtheta^{*}_\text{NN} ) + \log \frac{ p(\vy_i|\vtheta_\text{PGM})}{ q(\vx_n|\vy_n, \vphi_\text{NN}) } \bigg\rvert_{\vphi= \vphi^{*}  }  $
%
%\STATE Update gradient w.r.t. $\vphi$ due to additional terms in SIN
%
%$\vg_{\phi} \leftarrow  \nabla_{\phi } \sqr{-\log p(\vx^{*}_n | \vphi_\text{PGM}) + \log \mathcal{Z}(\vphi) } \bigg\rvert_{\vphi= \vphi^{*}  } $
%
%\STATE Perform adaptive-gradient update
%
%$\vg \leftarrow \sqr{  \vg_{ \theta_\text{NN} }, \vg_{\phi} }$,
%$\vmu \leftarrow \sqr{  \vmu_{ \theta_\text{NN} }, \vmu_{\phi} }$,
%$\vsigma^{-2} \leftarrow \sqr{  \vsigma^{-2}_{ \theta_\text{NN} }, \vsigma^{-2}_{\phi} }$
%
%$\vsigma^{-2} \leftarrow \vsigma^{-2} + \beta \vg \odot \vg$
%
%$\vmu \leftarrow \vmu + \beta \vsigma^{2} \odot \vg $
%
%    \ENDFOR
%\end{algorithmic}
%\end{algorithm}






%The only issue we need to solve is to make CVI applicable to the deterministic global parameters $\vdtrmc = \{\vmodlNN, \vinfe\}$. 

%given that distribution $q(\vphi)$ is flexible enough. %What is more, the variational objective function is a valid lower bound of $L(\vphi)$.
%Therefore, instead of using SGD to maximize the lower bound $L(\vphi)$, we propose  to maximize the variational lower bound, $\myexpect_{q( \phi )} \sqr{ L( \vphi) }$. The mode of distribution $q( \vphi )$ recovers the optimal $\vphi$ for the original lower bound, $L(\vphi)$. By doing so, we can use CVI to update $q( \vphi )$. The reason is that we can marginalize out $\vlat$ and optimize $q( \vphi )$ instead. In this case, $q(\vlat| \text{NN}_{\phi})$ becomes a factor when we optimize $q( \vphi )$.
%
%We propose to use $q(\vphi)=\gauss(\vm_{\phi}, \vSigma_{\phi})$, where $\vSigma_{\phi}$ is a diagonal covariance matrix, and to maximize its variational objection function $\myexpect_{q(\phi)} \sqr{ L(\vphi) }$.  By doing so, we are able to apply CVI to update all parameters in the structured inference network. Because CVI is a generalization of variational message passing, our method automatically enables to perform variational message passing for the structured inference network.

%A final step to obtain our message-passing algorithm is the choice of the natural-gradient method. The approach of SVI only works for conjugate models, but the DNN likelihood in our network is non-conjugate. We will therefore use a method proposed by \cite{khan2017conjugate} which is a generalization of SVI. In this method, the messages for the conjugate part of the model reduces to SVI-like updates, but the messages for the rest of the model use stochastic-gradients.

%How can we combine these two different types of methods together? Ideally, we would like to compute stochastic gradients for the non-conjugate factors only and use closed-form updates for conjugate factors in the model. In this paper, we propose a method to do so. We will use the CVI method of \cite{khan2017conjugate} which is generalization of SVI and VMP to non-conjugate models.  CVI is  not only a mirror descent method but also a variational message passing method. Below, we give the CVI update for distribution $q(\vlat)$ given that we want to maximize $ \myexpect_{q(\lat)} \sqr { \log \frac{ \prod_{i} f_i(\vlat) }{q(\vlat)}  }  $
%\begin{align}
%\max_{\boldsymbol{\mu}} \,\, \ang{\vmu, \nabla_{\mu} \myexpect_{q(\lat)} \sqr { \log \frac{ \prod_{i} f_i(\vlat) }{q(\vlat)}  }   } - \frac{1}{\beta} \dkl{}{q(\vlat)}{q(\vlat_{ \text{old} })}  \label{eq:cvi}
%\end{align}
%When all factors  $f_i(\vlat)$ are conjugate, the solution of Eq. \ref{eq:cvi} is exactly the message passing update in VMP. (see. Alg 2. in  \cite{khan2017conjugate}).  If some factor $f_j(\vlat)$ is non-conjugate, the message for the factor is equal to the gradient  $\nabla_{\mu} \myexpect_{q(\lat)} \sqr { f_j(\vlat) }$.
%
%However, CVI can not apply to distribution, $q(\vlat| \text{NN}_{\phi})$, parameterized by NN, where outputs of the NN are parameters of $q(\vlat)$. The inference network in VAE is a case. The reason is that CVI directly updates the parameters of $q(\vlat)$. However, parameters of $q(\vlat)$ in the inference network are outputs of NN. A straightforward solution is update parameters of the NN, $\vphi$ by maximizing the lower bound $L(\vphi)$ (e.g., SGD).  In this paper, we propose to use an alternative solution which enables us to perform variational message passing in the structured inference network. What is more, we can show that our solution is also an adaptive gradient update for $\vphi$.
%We borrow the idea from variational optimization \citep{staines2012variational}. In variational optimization, it shows that the optimal solution $\vphi^{*}$ of  $L(\vphi)$ is the mode of the optimal distribution $q^{*}(\vphi)$ for the variational objective function $\myexpect_{q(\phi)} \sqr{ L(\vphi) }$. 
%%given that distribution $q(\vphi)$ is flexible enough. %What is more, the variational objective function is a valid lower bound of $L(\vphi)$.
%Therefore, instead of using SGD to maximize the lower bound $L(\vphi)$, we propose  to maximize the variational lower bound, $\myexpect_{q( \phi )} \sqr{ L( \vphi) }$. The mode of distribution $q( \vphi )$ recovers the optimal $\vphi$ for the original lower bound, $L(\vphi)$. By doing so, we can use CVI to update $q( \vphi )$. The reason is that we can marginalize out $\vlat$ and optimize $q( \vphi )$ instead. In this case, $q(\vlat| \text{NN}_{\phi})$ becomes a factor when we optimize $q( \vphi )$.
%
%We propose to use $q(\vphi)=\gauss(\vm_{\phi}, \vSigma_{\phi})$, where $\vSigma_{\phi}$ is a diagonal covariance matrix, and to maximize its variational objection function $\myexpect_{q(\phi)} \sqr{ L(\vphi) }$.  By doing so, we are able to apply CVI to update all parameters in the structured inference network. Because CVI is a generalization of variational message passing, our method automatically enables to perform variational message passing for the structured inference network.
%
%%We can show that CVI update in $q(\vphi)$ is an Adagrad-like update.  
%\comment{do we have to show the CVI update recovers an adagrad-like update}
%
%
%In variational optimization $\citep{staines2012variational}$, the mode of the optimal solution of $\vphi^{*}$ of the variational objective function $\myexpect_{q(\phi)} \sqr{ L(\vphi) }$

 %shows that when $q(\vphi)$ is flexible enough, the optimal solution $\vphi^{*}$ is the mode of $q(\vphi)$. Therefore, we propose to use $q(\vphi)=\gauss(\vm, \vSigma)$
%\begin{align}
%\vphi^{*} & = \arg \max_{\phi} L(\vphi) \\
%q^{*}(\vphi) &= \arg \max_{q} \myexpect_{q(\phi)} \sqr{ L(\vphi) }
%\end{align}




%However, CVI update can not apply to deterministic parameters, $\vphi$ (e.g., parameters of NN) because there is no variational distribution $q(\vphi)$ for $\vphi$. If we want to apply CVI to deterministic parameters, how can we do that?
  


  
%To correct this, we assume $q(\vphi)=\gauss(\vm_{\phi}, \vSigma_{\phi})$. Such correction is valid since it is an application of variational optimization \citep{staines2012variational}. It has been shown that the optimal mean $\vm_{\phi}$ of $q(\vphi)$ in the variational objective function recovers the optimal $\vphi$ in the original objective function. By doing so, we extend the CVI framework to handle deterministic parameters and are able to use CVI to update all parameters in SIN. Compared to black-box SGD, CVI is more efficient that SGD as shown in \cite{khan2017conjugate}.  




%In CVI, updates can be expressed in terms of message passing. For conjugate factor, message is available in close-form. For example, the CVI update recovers the SVI update for conjugate factor. For non-conjugate factor, message is expressed in terms of natural-gradient.




%Here, we give the CVI update for the lower bound as an example. Given the lower bound $L(\vphi, \vmu)$, the CVI update for $q(\vtheta|\vmu)$ is 
%\begin{align}
%\max_{\boldsymbol{\mu}} \,\, \ang{\vmu, \nabla_{\mu} \myexpect_{q} \sqr {  \log f_{\text{c}}(\vtheta) } +   \nabla_{\mu} \myexpect_{q} \sqr { \log f_{\text{nc}}(\vtheta) } } - \frac{1}{\beta} \dkl{}{q(\vtheta)}{q(\vtheta_{ \text{old} })} 
%\end{align}
%where  $q(\vtheta_{ \text{old} })$ denotes the distribution at the last iteration,  $\vmu_j$ is the mean parameter of distribution $q(\vlat_j)$.

%\comment{do we need to compute the gradient w.r.t. the normalizing constant ?}
%\comment{we need to define conditionally conjugatcy so that we can show the gradient w.r.t mean parameter is a closed-form }
 

% \max_{\boldsymbol{\mu_i}} \,\, \sum_{j \in  \mathcal{M}_i } \ang{\vmu_i, \nabla_{\mu_i} \log \frac{p(\vlat_j,\vlat_i)}{q(\vlat_i)} } - \frac{1}{\beta} \dkl{}{q(\vlat_i)}{q(\vlat_{i,t})}  

%Many of existing works use SGD to perform black-box update for the PGM factor, which in general ignores the structures of the PGM factor. Ideally, we want to use VMP update for the PGM factor and to use SGD update for the DNN factor in a principal way. Few existing works are able to perform such update.  


%We propose to extend the Conjugate-computation Variational Inference (CVI) \citep{khan2017conjugate} framework to SIN since CVI allows us to combine stochastic gradient and messaging passing. 

%CVI works well for generic PGM but can not apply to deterministic parameters such as parameters in NN. We will first review CVI and then extend CVI to handle deterministic parameters.   


%The CVI update can be viewed as message passing, where messages are expressed in terms of gradient with respect to mean parameter. \cite{khan2017conjugate} shows that when $p(\vlat_j,\vlat_i)$ is conjugate to $q(\vlat_i)$, $ \nabla_{\mu_i} \log \frac{p(\vlat_j,\vlat_i)}{q(\vlat_i)}$ reduces to the conjugate message in VMP. When it comes to non-conjugate $p(\vlat_j,\vlat_i)$, the gradient is used as the message from node $\vlat_j$ to node $\vlat_i$. 

%CVI update can not apply to deterministic parameters, $\vphi$ because there is no variational distribution  $q(\vphi)$.  To correct this, we assume $q(\vphi)=\gauss(\vm_{\phi}, \vSigma_{\phi})$. Such correction is valid since it is an application of variational optimization \citep{staines2012variational}. It has been shown that the optimal mean $\vm_{\phi}$ of $q(\vphi)$ in the variational objective function recovers the optimal $\vphi$ in the original objective function. By doing so, we extend the CVI framework to handle deterministic parameters and are able to use CVI to update all parameters in SIN. Compared to black-box SGD, CVI is more efficient that SGD as shown in \cite{khan2017conjugate}.
  




%\subsubsection{Variational Mixture of Gaussians}
%The variational EM-algorithm described in \citet{bishop2006pattern} is such method to perform variational inference in a 'simple' GMM 
%\begin{align}
%	p(\vy) = \prod_{k=1}^K\pi_k^{z_{nk}}\gauss(\vy\given\vmu_k,\vSigma_k)^{z_{nk}},
%\end{align}
%which corresponds to the PGM-part of our model.
%
%The cojugate prior distribution over the model parameters $p(\vtheta) = p(\vpi)p(\vmu,\vSigma)$ used is composed of a Dirichlet distribution $p(\vpi) = \Dir(\vpi\given\valpha_0)$ with parameter $\valpha_0$ and a normal-Wishart distribution $p(\vmu,\vSigma) = \prod^K_{k=1}\gauss(\vmu_k\given\vm_0, \frac{1}{\beta_0}\vSigma_k){\cal W}(\vSigma_k^{-1}\given\vW_0,\nu_0)$ with parameters $\vm_0, \vbeta_0, \vW_0$ and $\nu_0$.
%
%In the M-step of this algorithm, the distribution $q^*(\vz)$, which is computed in the algorithm's E-step, is used for finding the variational distribution $q^*(\vtheta)$ by maximising the following lower bound (cf. eq. 10.6 in  \citet{bishop2006pattern}):
%\begin{align}
%	\elbofinal_{GMM} 
%		&= \int q\rnd{\vtheta} \rnd{ \int \log{ p\rnd{\vy, \vz, \vtheta} } q^*\rnd{\vz} d\vz }
%		d\vtheta 
%			- \int q\rnd{\vtheta} \log{q\rnd{\vtheta}} d\vtheta 
%			+ \text{const}  \nonumber \\
%		&= \myexpect_{q\rnd{\theta} q^*\rnd{z}} \sqr{ \log{p\rnd{\vy,\vz\given\vtheta}}} 
%			- \dkls{} {q\rnd{\vtheta}} {p\rnd{ \vtheta }} 
%			+ \text{const}  \nonumber \\
%		&= \myexpect_{q\rnd{\theta} q^*\rnd{z}} \sqr{ \sum^N_{n=1}\sum^K_{k=1} z_{nk} \log{ \pi_k \gauss\rnd{\vy_n\given\vmu_k, \vSigma_k} }} 
%			- \dkls{} {q\rnd{\vtheta}} {p\rnd{ \vtheta }} 
%			+ \text{const}  \nonumber \\
%		&= \sum^N_{n=1} \sum^K_{k=1} r_{nk} \log{\rho_{nk}}
%			- \dkls{} {q\rnd{\vtheta}} {p\rnd{ \vtheta }} 
%			+ \text{const}, \label{eq:ELBO-bishop}
%\end{align}
%where $r_{nk} = \myexpect_{q^*\rnd{z}}\sqr{z_{nk}}$ is the mean parameter of $q^*(z_{nk})$ and
%\begin{align}
%	\log{\rho_{nk}} &= \myexpect_{q(\pi)}\sqr{\log{\pi_k}} - \frac{D}{2}\log{2\pi} - \frac{1}{2}\myexpect_{q(\mu,\Sigma)}\sqr{\log{\left|\vSigma_k\right|} + \rnd{\vy_n - \vmu_k}^T\vSigma^{-1}\rnd{\vy_n - \vmu_k}}.
%\end{align}
%
%The following derivation shows that for updating our parameter $\vmodlGM$, we optimise a lower bound very similar to \ref{eq:ELBO-bishop}. The terms in our lower bound (eq. \ref{eq:elbo}) that involve parameter $\vmodlGM$ can be written as follows:
%\begin{align}
%\overline{\elbofinal}_{PGM}
%	&= \myexpect_{q(\phi)q_\phi(x,z|y)q(\modlGM)} \sqr{ \log p(\vx,\vz \given \vmodlGM) } - \dkls{} {q\rnd{\vmodlGM}} {p\rnd{ \vmodlGM }}  \nonumber \\
%	&=  \myexpect_{q(\modlGM)q_{\phi^*}(z_n|y_n)} \sqr{ 
%			\sum^N_{n=1} \sum^K_{k=1} z_{nk} \log{ \pi_k \gauss(\vx_n^* | \vmu_k, \vSigma_k) } }
%		- \dkls{} {q\rnd{\vmodlGM}} {p\rnd{ \vmodlGM }}  \nonumber
%	\\
%	&= \sum^N_{n=1} \sum^K_{k=1} \overline{r}_{nk} \log{\overline{\rho}_{nk}} 
%		- \dkls{} {q\rnd{\vmodlGM}} {p\rnd{ \vmodlGM }}\label{eq:elbo-GMM-as-Bishop} ,
%\end{align}
%where
%\begin{align}
%	\log{\overline{\rho}_{nk}} &= \myexpect_{q(\pi)}\sqr{\log{\pi_k}} - \frac{D}{2}\log{2\pi} - \frac{1}{2}\myexpect_{q(\mu,\Sigma)}\sqr{\log{\left|\vSigma_k\right|} + \rnd{\vx^*_n - \vmu_k}^T\vSigma^{-1}\rnd{\vx^*_n - \vmu_k}}.
%\end{align}
%
%We see that our update of $q(\vmodlGM)$ differs from the M-step of the variational GMM-EM algorithm in that it makes use of the structured recognition model: We compute $\log{\overline{\rho}_{nk}}$ using the sampled $\vx^*_n$ instead of the data $\vy_n$ and our responsibilities $\overline{r}_{nk}$ are computed using $q_{\phi^*}(z_n|y_n)$, as explained in section \ref{sec:e-step}. Due to this similarity, we can apply the M-step proposed by \citet{bishop2006pattern}, i.e., we use the same prior distribution and apply the same closed-form updates for computing $q(\vtheta, \vlambda^*_\theta)$ (cf. eq.10.57 - 10.63 in \citet{bishop2006pattern}). Then, we perform a CVI update by computing a convex combination of the current and the updated distribution
%\begin{align}
%	q\rnd{\vtheta|\lambda_{\theta_{t+1}}} = q\rnd{\vtheta|\lambda_{\theta_{t}}}^{1-\beta_t} q(\vtheta, \vlambda^*_\theta)^{\beta_t}
%\end{align}


==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

